Bending laminations on convex hulls of anti-de Sitter quasicircles

Let $\lambda_-$ and $\lambda_+$ be two bounded measured laminations on the hyperbolic disk $\mathbb H^2$, which "strongly fill" (definition below). We consider the left earthquakes along $\lambda_-$ and $\lambda_+$, considered as maps from the universal Teichm\"uller space $\mathcal T$ to itself, and we prove that the composition of those left earthquakes has a fixed point. The proof uses anti-de Sitter geometry. Given a quasi-symmetric homeomorphism $u:{\mathbb RP}^1\to {\mathbb RP}^1$, the boundary of the convex hull in $AdS^3$ of its graph in ${\mathbb RP}^1\times{\mathbb RP}^1\simeq \partial AdS^3$ is the disjoint union of two embedded copies of the hyperbolic plane, pleated along measured geodesic laminations. Our main result is that any pair of bounded measured laminations that "strongly fill" can be obtained in this manner.

==> laminations3old.tex <==
\section{Ideal polyhedra and approximation of laminations.} %% JMS

In this section, we show how to approximate a pair of measured laminations that strongly fill in $\HH^2$ by a sequence of pairs of ``polyhedral'' laminations, that is, measured laminations on ideal polygons with support contained in a union of disjoint diagonals. We first define what we mean by a ``polyhedral'' measured lamination on $\HH^2$.

\begin{defi}
  A measured lamination on $\HH^2$ is {\em polyhedral} if its support is the disjoint union of a finite set of complete geodesics.
\end{defi}

\begin{defi}
  Let $P$ be an idea polyhedron in $AdS^3$, and let $P_-$ and $P_+$ be its past and future boundary components.\marginnote{JM: vérifier que c'est défini dans la section 2.}
  Each of those two pleated ideal polygons defines a polyhedral measured lamination. We denote these two laminations by $\lambda_-(P)$ and $\lambda_+(P)$ respectively.
  We denote by $V(P)$ the $n$-tuple of vertices of $P$, cyclically oriented in the order in which they occur on any acausal meridian containing them. 
\end{defi}

By construction, $\lambda_\pm(P)$ have a support which is a disjoint union of diagonals, that is, complete geodesics connecting two vertices. 

\begin{theorem}
Let $\lambda_-$, $\lambda_+\in \cML$ be a pair of laminations that strongly fill.
There exists a sequence $(P_n)_{n\in \N}$ of ideal polyhedra and a sequence $u_n$ of functions from $V(P_n)$ to $\RP^1$ such that $((u_{n})_*(\lambda_-(P_n)))_{n\in \N}$ and $((u_{n})_*(\lambda_+(P_n)))_{n\in \N}$ converge to $\lambda_-$ and $\lambda_+$, respectively.
\end{theorem}

The convergence considered here is in the sense of weak-$*$ convergence on measures in $\RP^1\times \RP^1\setminus \Delta$.\marginnote{JM: vérifier, c'est bien ça ?}


\begin{proof}
Let us first construct a weighted spherical graph out of which we will get a polyhedron using the main result of \cite{idealpolyhedra}. 

We fix $n\in\mathbb{N}$ and we consider the disk $D(o,n)$ of radius $n$ centered at a fixed point $o\in\mathbb{H}^2$ . We remove from $\lambda_-$ and $\lambda_+$ the leaves which does not intersect $D(o,n)$. We denote those truncated laminations by $\lambda_-^n$ and $\lambda_+^n$; our aim is to approximate them by polyhedral laminations. The total weight of those truncated lamination is finite, it equals twice the sum of the intersections of the circle $C(o,n)$ with the laminations $\lambda_+$ and $\lambda_-$. We denote this total weight by $a_n$.

We now arrange $k$ points on the circle $\mathbb{S}^1=\partial_\infty\mathbb{H}^2$ according to the following procedure. The number $k$ will be chosen later as a function of $n$. We use the Poincaré disk model of $\mathbb{H}^2$. We first set $a_1=i$. Assuming that $a_j$ has been constructed, we construct $a_{j+1}$ in such a way that the leaves of $\lambda_-^n$ and $\lambda_+^n$ limiting in the interval $\left[a_ja_{j+1}\right)$ have a total weight of $\frac{a_n}{k}$. If a single leaf carries too much weight, we divide it into parallel geodesics and we fairly split the weights. This defines $k$ points on $\mathbb{S}^1$.


We now describe a weighted graph $\Gamma$ which encodes the 1-skeleton and exterior dihedral angles of polyhedron we are looking for.
\begin{enumerate}
\item $\Gamma$ has a vertex $v_j$ in each segment $\left[a_ja_{j+1}\right)$.
\item Two vertices $v_j$ and $v_{j'}$ are related by an edge whose weight is the total weight of the leaves of $\lambda_-^n$ (resp. $\lambda_+^n$) from the interval $\left[a_ja_{j+1}\right)$ to $\left[a_{j'}a_{j'+1}\right)$, if there is any such leave.
\item The adjacent vertices $v_j$ and $v_{j+1}$ are related by an edge of weight $-\frac{a_n}{2k}$.
\end{enumerate}
Given an edge $e$ of this graph, we denote by $\theta(e)$ its weight.


\begin{lemma}
The weighted graph $\Gamma$ satisfies the hypothesis of \cite[Theorem 1.4]{idealpolyhedra} for $k$ large enough.
\end{lemma}

\begin{proof}
The fact that the graph has a Hamiltonian circle is obvious. The link condition is also trivially satisfied. We need to show is that if $e^*_1,e^*_2,\cdots, e^*_q$ is a closed path in the dual graph $\Gamma^*$ which does not bound a face of $\Gamma^*$ but intersect exactly two edges of the ``equator'' (edges of $\Gamma$ with negative weight), then\marginnote{JM: rewritten. No reason why $p=q$, right?}
\[\sum_{i=1}^q\theta(e^*_i)>0.\]
This issue reduces\marginnote{JM: ok but we need to explain why.} to the following statement: let $\gamma$ be a geodesic path in $\mathbb{H}^2$ connecting the interval $\left(v_1v_2\right)$ to $\left(v_{p}v_{p+1}\right)$. Then the total weight of the edges of $\lambda_-^n$ and $\lambda_+^n$ it crosses is bigger than $\frac{a_n}{k}$. We argue differently according to the relative position of $v_1$ and $v_p$.

\textbf{1st case:} The path $\gamma$ does not enter the disk $D(o,n)$. Since each edge of $\lambda_\pm$ enters $D(o,n)$, $\gamma$ must cross all the edges emanating from $v_2$ and $v_p$, for a total weight of $\frac{2a_n}{k}$.


\definecolor{ttttff}{rgb}{0.2,0.2,1}
\begin{figure}[!h]
\begin{tikzpicture}[scale=0.8][line cap=round,line join=round,>=triangle 45,x=1.0cm,y=1.0cm]
\clip(-5.87,-13.42) rectangle (34.33,8.12);
\draw [shift={(10.38,-2.32)}] plot[domain=1.68:4.33,variable=\t]({1*9.01*cos(\t r)+0*9.01*sin(\t r)},{0*9.01*cos(\t r)+1*9.01*sin(\t r)});
\draw [shift={(10.7,-2.28)}] plot[domain=1.94:4.24,variable=\t]({1*7.88*cos(\t r)+0*7.88*sin(\t r)},{0*7.88*cos(\t r)+1*7.88*sin(\t r)});
\draw [shift={(-35.65,-237.6)}] plot[domain=1.37:1.41,variable=\t]({1*241.03*cos(\t r)+0*241.03*sin(\t r)},{0*241.03*cos(\t r)+1*241.03*sin(\t r)});
\draw [shift={(-5.95,-77.88)}] plot[domain=1.33:1.47,variable=\t]({1*76.84*cos(\t r)+0*76.84*sin(\t r)},{0*76.84*cos(\t r)+1*76.84*sin(\t r)});
\draw [shift={(2.7,3.55)}] plot[domain=-1.85:0.55,variable=\t]({1*3.18*cos(\t r)+0*3.18*sin(\t r)},{0*3.18*cos(\t r)+1*3.18*sin(\t r)});
\draw [shift={(7,6.27)}] plot[domain=-2.55:0.12,variable=\t]({1*1.91*cos(\t r)+0*1.91*sin(\t r)},{0*1.91*cos(\t r)+1*1.91*sin(\t r)});
\draw [shift={(1.37,-3.65)}] plot[domain=-1.26:1.55,variable=\t]({1*2.26*cos(\t r)+0*2.26*sin(\t r)},{0*2.26*cos(\t r)+1*2.26*sin(\t r)});
\draw [shift={(2.87,-7.77)}] plot[domain=-0.7:1.96,variable=\t]({1*2.13*cos(\t r)+0*2.13*sin(\t r)},{0*2.13*cos(\t r)+1*2.13*sin(\t r)});
\draw [line width=1.6pt,color=ttttff] (1.41,-1.39)-- (2.85,-1.54);
\draw (6.71,-8.26) node[anchor=north west] {$D(0,n)$};
\draw (4.27,-9.47) node[anchor=north west] {$ \partial_\infty \mathbb{H}^2 $};
\draw (2.28,-0.71) node[anchor=north west] {$ \lambda_0 $};
\draw (6.91,-1.39) node[anchor=north west] {$\partial_r b^+$};
\draw [shift={(1.35,-0.39)}] plot[domain=-1.51:1.09,variable=\t]({1*1*cos(\t r)+0*1*sin(\t r)},{0*1*cos(\t r)+1*1*sin(\t r)});
\draw (2.26,0.43) node[anchor=north west] {$\partial_0 b^+$};
\draw (7.73,0.28) node[anchor=north west] {$\partial_l b^+$};
\draw (5.6,2.75) node[anchor=north west] {$\partial B^+$};
\end{tikzpicture}
\label{fig:notation}
\caption{Notations used in the approximation procedure.}
\end{figure}


\textbf{2nd case:} The geodesic $\gamma$ does enter the disk $D(0,n)$. Note that the case where the path enter $D(0,n)$ for a length at least $c$ corresponding to $\varepsilon=\frac{2a_n}{k}$ in the definition of the strong filling condition is easily taking care of by the strong filling hypotheses. Nevertheless, the following argument also handles the case where the intersection of $\gamma$ and $D(0,n)$ is short. We will use the following notations (see figure \ref{fig:notation}). We denote by $B^+$ and $B^-$ the polygons corresponding to the union of the faces that $\gamma$ meets in the dual graph of $\lambda_n^+$ and $\lambda_n^-$ respectively. We also consider the quadrilateral $b$ which is the convex hull of the boundary edges crossed by $\gamma$, i.e in the above notations the edges $\left(v_1v_2\right)$ and $\left(v_{p}v_{p+1}\right)$ and we denote by $b^+$ and $b^-$ the two copies of $b$ in the upper and lower side. Then $\partial_r b^+$ and $\partial_l b^+$ are the remaining sides of $b^+$ (same for $b^-$). Finally $\lambda_0$ is the part of $\partial_r b^+$ lying outside $D(0,n)$.
\end{proof}

The fact that $\lambda_+(P_n)$ converge to $\lambda_+$ and $\lambda_-(P_n)$ converge to $\lambda_-$ follows directly from the definition of the topology on $\cML$. \note{good ref}

\end{proof}

We now associate to those truncated laminations, an approximation of the quasi-circle we are looking for. Indeed, let $P_n$ be the ideal polyhedra we constructed in the previous theorem. With its Hamiltonian path, we connect all of its vertices by a path $v^n:\mathbb{RP}^1\rightarrow \partial_\infty$AdS$^3$ which is piecewise $\mathcal{C}^1$ with breaking points only at the vertices and with left and right derivatives everywhere. Moreover we take $v^n$ uniformly acausal in the sense that its (left and right) tangent are uniformly far from a lightlike line. This later condition rephrases as $v^n$ being quasi-symmetric. \marginnote{JM: je ne vois pas bien pourquoi, il me semble qu'il manque une preuve.}

==> laminations4.new.tex <==
\section{Proof of Theorem \ref{tm:bending}.} %% JMS

We now come to the proof of the main theorem. 

\subsection{Discrete approximations of quasi-symmetric homeomorphisms}

We first introduce a simple notion of quasi-symmetry for maps from a finite subset of $\RP^1$ to $\RP^1$.\marginnote{JM: En fait je pense qu'on peut prendre $\epsilon$ fixé, par exemple 1/2, dans toute la section.}

\begin{defi}
  Let $F\subset \RP^1$ be a finite subset, and let $v:F\to \RP^1$ be an increasing map. Let $\epsilon>0, K>1$. We say that $v$ is $(K,\epsilon)$-quasisymmetric if for all $a,b,c,d\in F$ with $[a,b;c,d]\in [-1-\epsilon,-1+\epsilon]$, $[v(a),v(b); v(c),v(d)]\in [1/K,K]$. \marginnote{L: changed 2 into -1}
\end{defi}

In the sequel, we say that  $a,b,c,d\in \mathbb{RP}^1$ with $[a,b;c,d]\in [-1-\epsilon,-1+\epsilon]$ are in $\epsilon$-symmetric position.

Clearly, if $v:\RP^1\to \RP^1$ is a $K$-quasi-symmetric homeomorphism, then the restriction of $v$ to any finite subset of $\RP^1$ is $(K',\epsilon)$-quasi-symmetric for some $\epsilon>0$, for a $K'$ depending on $K$ and $\epsilon$. \marginnote{JM: faudrait ajouter une preuve.}

Conversely, if a sequence of discrete uniformly quasi-symmetric homeomorphisms converges to a limit, it must be quasiconformal.

\begin{lemma} \label{lem:limit}
  Let $u:\RP^1\to \RP^1$ be a continuous map, and let $(F_n,v_n)_{n\in \N}$ be a sequence of pairs such that:
  \begin{itemize}
  \item for all $n$, $F_n\subset \RP^1$ is a finite subset, and for all $x\in \RP^1$, there exists a sequence $(x_n)_{n\in \N}$, with $x_n\in F_n$, such that $x_n\to x$,
  \item $v_n\to u$, in the sense that if $x_n\in F_n$ and $x_n\to x$ then $v_n(x_n)\to u(x)$,
  \item the $v_n$ are $(K,\epsilon)$-quasisymmetric, for fixed $K>1$ and $\epsilon>0$.  
  \end{itemize}
  Then $u$ is $K$-quasisymmetric. \marginnote{L: changed, ok ?}
\end{lemma}

\begin{proof}
Let $a,b,c,d$ be 4 points in $\mathbb{RP}^1$ in symmetric position. There exists 4 sequences $(a_n), (b_n), (c_n)$ and $(d_n)$ converging to $a,b,c$ and $d$ respectively. Since the cross-ratio is a continuous function, for $n$ big enough, the 4 points $a_n,b_n,c_n$ and $d_n$ are in $\varepsilon$-symmetric position. It followsWe get that $[v(a_n),v(b_n); v(c_n),v(d_n)]\in [1/K,K]$. The result follows from the definition of $u$ and continuity of the cross-ratio.
\end{proof}

Finally we can state a kind of compactness result for $(K,\epsilon)$-quasisymmetric maps.

\begin{lemma}\label{lem:precompactness}
  Let $K>1, \epsilon>0$, and let $(F_n,v_n)$ be a sequence of pairs, where
  \begin{enumerate}
  \item for each $n$, $F_n$ is a finite subset of $\RP^1$, and for all $x\in \RP^1$, there exists a sequence $(x_n)_{n\in \N}$, with $x_n\in F_n$, such that $x_n\to x$,
  \item the $v_n$ are $(K,\epsilon)$-quasisymmetric.
  \end{enumerate}
  Then there exists a subsequence of $(F_n, v_n)$ converging to a limit $u$ in the sense of Lemma \ref{lem:limit}.
\end{lemma}

This limit $u$ is then quasisymmetric by Lemma \ref{lem:limit}.

\begin{proof}
Without loss of generality, we can assume that $n$ is big enough so that $F_n$ has at least three points. Since pre and post composing by a Mobiüs transformation does not change the fact that $v_n$ is $(K,\epsilon)$-quasi-symmetric, we can assume that the points $0,-1,\infty\in\mathbb{RP}^1$ are sent to $0,-1,\infty$ respectively.

Since $\mathbb{RP}^1$ is compact, we know that $(F_n,v_n)$ have a converging subsequence. Indeed, Arzela-Ascoli theorem applies to the set of maps $v_n:F_n\rightarrow \mathbb{RP}^1$ for a fixed $n$ and then the set of all sequences $(F_n,v_n)$ is relatively compact by Tychonoff's theorem. We denote by $u$ this sublimit. It is defined on the whole $\mathbb{RP}^1$ because of hypothesis (1). The goal is to show that $u$ is a homeomorphism of $\mathbb{RP}^1$ onto itself. Note that $u$ also satisfies $u(-1)=-1$, $u(0)=0$ and $u(\infty)=\infty$.

By lemma \ref{lem:limit}, $u$ is $K$-quasi-symmetric (i.e the images of 4 points in symmetric position have a bounded cross-ratio) and non-decreasing. We first show that $u$ is continuous. By contradiction, assume that $u$ has a "jump" at $x\in\mathbb{RP}^1$: there exists a sequence $y_n$ converging to $x$ such that, for a fixed $\delta$, $\abs{u(x)-u(y_n)}>\delta$. Take any point $z\in\mathbb{RP}^1$, $z\neq x$. There exists a sequence $(t_n)$ such that $[x,y_n;z,t_n]=-1$ (in particular $t_n\to z$) and $[u(x),u(y_n);u(z),u(t_n)]$ is bounded. Hence $u(t_n)$ cannot approach $u(z)$. Since $u$ is non-decreasing, what is true for $(t_n)$ is also true in a whole neighborhood of $z$. We conclude that $u(z)$ is isolated in $u(\mathbb{RP}^1)$. Since $z$ was chosen arbitrarily (different from $x$), this means that $u$ has at most 2 values, contradicting the fact that $u(-1)=-1$, $u(0)=0$ and $u(\infty)=\infty$.


Finally, we show that $u$ is injective using the same kind of argument. Assuming that $u(x)=u(y)$, we take any $z\in\mathbb{RP}^1$ and find the point $t\in\mathbb{RP}^1$ such that $\crochet{x,y;z,t}=-1$. For $\crochet{u(x),u(y);u(z),u(t)}$ to remain bounded, we must have $u(z)=u(t)$ and then again, $u$ has only 2 values.

\end{proof}

\subsection{The discrete approximations are uniformly quasi-symmetric.}



Recall that we started with a pair $(\lambda_-, \lambda_+)$  of laminations on $\HH^2$ that strongly fill. We associated to this pair:
\begin{itemize}
\item sequences $\lambda^n_\pm=\lambda^n_\pm$ of polyhedral pairs converging to $\lambda_\pm$, with $k_n$ vertices, and
\item a sequence of quasi-symmetric embeddings $v^n:\Z/k_n\Z\to\partial_\infty AdS^3$ such that $v^n_*(\lambda^n_\pm)$ are the measured bending laminations on the boundary of $CH(v^n(Z/k_n\Z))$.
\end{itemize}
%% We denote by $C_n=v^n(\mathbb{RP}^1)$. 

We then have a sequence of pairs of convex isometric embeddings $U^n_\pm:P^n_\pm\to AdS^3$, where $P^n_\pm$ are ideal polygons in $\HH^2$ with $k_n$ vertices, with images the upper and lower boundary components of $CH(v^n(\Z/k_n\Z))$. If we denote by $V_n$ the set of vertices of $P_\pm^n$ in $\partial_\infty\mathbb{H}^2$, we also consider the map $u^n_\pm=\partial U^n_\pm:V_n\subset \mathbb{RP}^1\rightarrow \partial_\infty AdS^3$. Those maps $u_\pm^n$ are injective and then have a left inverse $\left(u_\pm^n\right)^{-1}: \partial_\infty AdS^3\rightarrow \mathbb{RP}^1$. 



% In order to apply \ref{lem:precompactness}, we need to show that the discrete maps $\left(u_\pm^n\right)^{-1}\circ v^n : \Z/k_n\Z \rightarrow \mathbb{RP}^1$ are \textit{uniformly} $(K,\epsilon)$-quasi-symmetric, in the sense of the previous paragraph. This is the point of the next lemma, whose proof uses decisively the fact that the laminations $\lambda^\pm$ are bounded.
% %We know that the set of \textit{uniform} quasi-symmetric embeddings is compact \cite{lehtovirtanen}. That should be the main argument to obtain the quasi-circle. The uniform quasi-symmetric constants should in term follow from a uniform bound on the width on $C_n$:

% \begin{lemma}
% There exist $\epsilon>0$ and $K>1$ such that, for $n$ big enough, the maps $\left(u_\pm^n\right)^{-1}\circ v^n : \Z/k_n\Z \rightarrow \mathbb{RP}^1$ are $(K,\epsilon)$-quasi-symmetric.
% \end{lemma}

% \begin{remark}
% In fact we can show the following equivalences ...\marginnote{L: I'm thinking of removing completely the width, even in the preliminaries}
% \end{remark}

% \begin{proof}
% We argue by contradiction and we assume that the maps $f^n=\left(u_\pm^n\right)^{-1}\circ v^n$ are $(K_n,\varepsilon)$-quasi-symmetric with $K_n\to \infty$. We then have four sequences $(a_n), (b_n), (c_n)$ and $(d_n)$ in $\mathbb{RP}^1$ such that $\crochet{a_n,b_n;c_n,d_n}\in \crochet{1-\epsilon,1+\epsilon}$ and $\crochet{f^n(a_n),f^n(b_n);f^n(c_n),f^n(d_n)}\to 0$ (the case where $\crochet{f^n(a_n),f^n(b_n);f^n(c_n),f^n(d_n)}\to \infty$ is similar). Pre and post-composing by a Mobiüus map does not chnage the quasi-symmetry constant $K_n$. Hence, we may as well assume that $f^n$ sends $a_n=0,b_n=-1,c_n=\infty$ to $0,-1,\infty$ respectively and $f^n(d_n)$ converges to 0 (the normalization forces $d_n$ to be in the interval $\crochet{1-\epsilon, 1+\epsilon}$). We now (post) compose $f^n$ by a Mobiüs map $\gamma_n$ and we chose $\gamma_n$ such that it is a hyperbolic transformation whose repuslive fixed point is 0 and attractive fixed point is $\infty$. Representing $\gamma_n$ by a matrix in SL$_2(\mathbb{R})$, $\gamma_n$ has the form
% \[
% \gamma_n=\begin{pmatrix}
% e^{\alpha_n} & 0\\
% 0 & e^{-\alpha_n}
% \end{pmatrix},
% \]
% with $\alpha_n>0$ and $\alpha_n\to \infty$.
% We want to choose the rate of attraction/repulsion $\alpha_n$ so that it provides a contradiction. We say that two sequences $(\alpha_n)$ and $(\alpha'_n)$ are uncomparable if either $\frac{\alpha_n}{\alpha'_n}\to 0$ or $\frac{\alpha_n}{\alpha'_n}\to +\infty$. Note that there is infinitely many uncomparable sequences and we will choose the sequence $\alpha_n$ among finitely many constraints.

% First we require that $f^n\circ \gamma_n (d_n)$ tends to 0 and $f^n\circ\gamma_n(-d_n)$ tends to 0. Then, if we denote by $d_n^+$ the element of $ \Z/k_n\Z $ which is the successor of $d_n$ for the cyclic order on $\mathbb{RP}^1$ and $d_n^-$ the predecessor of $-d_n$ we choose $\alpha_n$ in such a way that $f^n\circ \gamma_n(d_n^-)$ and $f^n\circ \gamma_n (d_n^+)$ both tend to $\infty$.

% Since the maps $f^n$ are increasing, we get that any element $x_n\in  \Z/k_n\Z $ which is in the interval $\crochet{-d_n,d_n}$ containing 0 satisfies $f^n\circ \gamma_n(x_n) \rightarrow 0$ and any element $x_n\in  \Z/k_n\Z $ in the interval $\crochet{d_n,-d_n}$ containing $\infty$ satisfies $f^n\circ \gamma_n(x_n)\rightarrow \infty$.

% We conclude that the maps $u^n_\pm$ converge to the Rhombus curve constructed with the four points $a=-1, a'=1, b=\infty, b'=0$ (referring to the notation of paragraph \ref{subsec:rhombus}). The rhombus has two space-like geodesics inside $AdS^3$. Those geodesics bound lightlike planes and then both have an infinite dihedral angle, contradicting lemma \ref{lem:reciprocalbounds}.
% \end{proof}


% %\begin{lemma}
% %The convex subsets $CH(v_n(\Z/k_n\Z))$ have width bounded away from $\frac{\pi}{2}$ (independent of $n$).
% %\end{lemma}

% %The proof is similar to one given, in a simular situation, in e.g. \cite{convexhull}.

% %\begin{proof}
% %  (outline)
  
% %  (1) If not then after applying sequence of isometries, $x_-, x_+$ at time distance $\pi/2$.

% %  (2) Support lines at $x_-$ and $x_+$, must be dual to each other because acausal meridian joining the vertices.

% %  (3) The total bending near those two lines must go to infinity.

% %  (4) Take four points $a,b,c,d$ separating the endpoints, e.g. vertices.

% %  (5) Apply Lemma \ref{lem:reciprocalbounds}.
% %\end{proof}

% % \begin{proof}
% % If not, the convex hull eventually (as $n\to\infty$) contains a rhombus.The rhombus has two space-like geodesics inside $AdS^3$. Those geodesics bound  lightlike planes and then both have an infinite dihedral angle, contradicting lemma \ref{lem:reciprocalbounds}.
% % \end{proof}


% %\subsection{The discrete approximations are uniformly quasi-symmetric}






% \begin{lemma}
% $(u^n_-)^{-1}\circ u^n_+$ is uniformly quasi-symmetric.
% \end{lemma}

% \begin{proof}
  
% \end{proof}

% %% NB the argument below might be useful, but they don't seem to be necessary.
% % \begin{proof}
% % Should follow from the fact that the projection \note{ref} from the upper to the lower boundary is a uniform quasi-isometry (which in turns should follow from the bound on the width).
% % \end{proof}


% %\begin{lemma}
% %The homeomorphisms $(u^n_\pm)^{-1}\circ v^n$ are uniformly quasi-symmetric.
% %\end{lemma}


% %\begin{proof}
% %We only treat the case of $(u^n_+)^{-1}\circ v_n$, the other one is obviously the same.
% %We argue by contradiction and we suppose that the $(u^n_+)^{-1}\circ v_n$ are not uniformly quasi-symmetric. Then (?? check ??) there is a sequence of 4-tuples of points $(a_n,b_n,c_n,d_n)$ with images $(a'_n, b'_n, c'_n,d'_n)$ such that $cr(a_n,b_n,c_n,d_n)\geq n$ and $cr(a'_n,b'_n,c'_n,d'_n)\leq 1/n$. Because of the strong filling hypothesis, we can also assume for instance that $\lambda^n_+([a_n,b_n]\times [c_n,d_n])\geq n\epsilon/2$ (after extracting a subsequence). Indeed, choosing one of the two laminations, we can assume that $\lambda^n_+([a_n,b_n]\times [c_n,d_n])$ is the intersection number of a geodesic joining the arc $[a_n,d_n]$ to the arc $[b_n,c_n]$ which has length proportional to $n$. Then the upper boundary has bending measure going to $\infty$ near the geodesic which is the limit of the image of $(a'_n,b'_n)$ and $(c'_n, d'_n)$. Contradiction (with the fact that we don't have a "rhombus" in the limit.)
% %\end{proof}

% \subsection{Proof of Theorem \ref{tm:bending}}

% Thanks to the lemma we can assume (after taking a subsequence and normalizing by M\"obius transformations) that the $(u^n_\pm)^{-1}\circ v^n$ are converging to quasi-symmetric homeomorphisms. It should then follow that the sequence of convex pleated surfaces converge and that the bending lamination on the boundary converges to $\lambda_+, \lambda_-$.

==> laminations4.old.tex <==
\section{Proof of Theorem \ref{tm:bending}.} %% JMS

We now come to the proof of the main theorem. 

\subsection{Discrete approximations of quasi-symmetric homeomorphisms}

We first introduce a simple notion of quasi-symmetry for maps from a finite subset of $\RP^1$ to $\RP^1$.\marginnote{JM: En fait je pense qu'on peut prendre $\epsilon$ fixé, par exemple 1/2, dans toute la section.}

\begin{defi}
  Let $F\subset \RP^1$ be a finite subset, and let $v:F\to \RP^1$ be an increasing map. Let $\epsilon>0, K>1$. We say that $v$ is $(K,\epsilon)$-quasisymmetric if for all $a,b,c,d\in F$ with $[a,b;c,d]\in [-1-\epsilon,-1+\epsilon]$, $[v(a),v(b); v(c),v(d)]\in [1/K,K]$. \marginnote{L: changed 2 into -1}
\end{defi}

In the sequel, we say that  $a,b,c,d\in \mathbb{RP}^1$ with $[a,b;c,d]\in [-1-\epsilon,-1+\epsilon]$ are in $\epsilon$-symmetric position.

Clearly, if $v:\RP^1\to \RP^1$ is a $K$-quasi-symmetric homeomorphism, then the restriction of $v$ to any finite subset of $\RP^1$ is $(K',\epsilon)$-quasi-symmetric for some $\epsilon>0$, for a $K'$ depending on $K$ and $\epsilon$. \marginnote{JM: faudrait ajouter une preuve.}

Conversely, if a sequence of discrete uniformly quasi-symmetric homeomorphisms converges to a limit, it must be quasiconformal.

\begin{lemma} \label{lem:limit}
  Let $u:\RP^1\to \RP^1$ be a continuous map, and let $(F_n,v_n)_{n\in \N}$ be a sequence of pairs such that:
  \begin{itemize}
  \item for all $n$, $F_n\subset \RP^1$ is a finite subset, and for all $x\in \RP^1$, there exists a sequence $(x_n)_{n\in \N}$, with $x_n\in F_n$, such that $x_n\to x$,
  \item $v_n\to u$, in the sense that if $x_n\in F_n$ and $x_n\to x$ then $v_n(x_n)\to u(x)$,
  \item the $v_n$ are $(K,\epsilon)$-quasisymmetric, for fixed $K>1$ and $\epsilon>0$.  
  \end{itemize}
  Then $u$ is $K$-quasisymmetric. \marginnote{L: changed, ok ?}
\end{lemma}

\begin{proof}
Let $a,b,c,d$ be 4 points in $\mathbb{RP}^1$ in symmetric position. There exists 4 sequences $(a_n), (b_n), (c_n)$ and $(d_n)$ converging to $a,b,c$ and $d$ respectively. Since the cross-ratio is a continuous function, for $n$ big enough, the 4 points $a_n,b_n,c_n$ and $d_n$ are in $\varepsilon$-symmetric position. It followsWe get that $[v(a_n),v(b_n); v(c_n),v(d_n)]\in [1/K,K]$. The result follows from the definition of $u$ and continuity of the cross-ratio.
\end{proof}

Finally we can state a kind of compactness result for $(K,\epsilon)$-quasisymmetric maps.

\begin{lemma}\label{lem:precompactness}
  Let $K>1, \epsilon>0$, and let $(F_n,v_n)$ be a sequence of pairs, where
  \begin{enumerate}
  \item for each $n$, $F_n$ is a finite subset of $\RP^1$, and for all $x\in \RP^1$, there exists a sequence $(x_n)_{n\in \N}$, with $x_n\in F_n$, such that $x_n\to x$,
  \item the $v_n$ are $(K,\epsilon)$-quasisymmetric.
  \end{enumerate}
  Then there exists a subsequence of $(F_n, v_n)$ converging to a limit $u$ in the sense of Lemma \ref{lem:limit}.
\end{lemma}

This limit $u$ is then quasisymmetric by Lemma \ref{lem:limit}.

\begin{proof}
Without loss of generality, we can assume that $n$ is big enough so that $F_n$ has at least three points. Since pre and post composing by a Mobiüs transformation does not change the fact that $v_n$ is $(K,\epsilon)$-quasi-symmetric, we can assume that the points $0,-1,\infty\in\mathbb{RP}^1$ are sent to $0,-1,\infty$ respectively.

Since $\mathbb{RP}^1$ is compact, we know that $(F_n,v_n)$ have a converging subsequence. Indeed, Arzela-Ascoli theorem applies to the set of maps $v_n:F_n\rightarrow \mathbb{RP}^1$ for a fixed $n$ and then the set of all sequences $(F_n,v_n)$ is relatively compact by Tychonoff's theorem. We denote by $u$ this sublimit. It is defined on the whole $\mathbb{RP}^1$ because of hypothesis (1). The goal is to show that $u$ is a homeomorphism of $\mathbb{RP}^1$ onto itself. Note that $u$ also satisfies $u(-1)=-1$, $u(0)=0$ and $u(\infty)=\infty$.

By lemma \ref{lem:limit}, $u$ is $K$-quasi-symmetric (i.e the images of 4 points in symmetric position have a bounded cross-ratio) and non-decreasing. We first show that $u$ is continuous. By contradiction, assume that $u$ has a "jump" at $x\in\mathbb{RP}^1$: there exists a sequence $y_n$ converging to $x$ such that, for a fixed $\delta$, $\abs{u(x)-u(y_n)}>\delta$. Take any point $z\in\mathbb{RP}^1$, $z\neq x$. There exists a sequence $(t_n)$ such that $[x,y_n;z,t_n]=-1$ (in particular $t_n\to z$) and $[u(x),u(y_n);u(z),u(t_n)]$ is bounded. Hence $u(t_n)$ cannot approach $u(z)$. Since $u$ is non-decreasing, what is true for $(t_n)$ is also true in a whole neighborhood of $z$. We conclude that $u(z)$ is isolated in $u(\mathbb{RP}^1)$. Since $z$ was chosen arbitrarily (different from $x$), this means that $u$ has at most 2 values, contradicting the fact that $u(-1)=-1$, $u(0)=0$ and $u(\infty)=\infty$.


Finally, we show that $u$ is injective using the same kind of argument. Assuming that $u(x)=u(y)$, we take any $z\in\mathbb{RP}^1$ and find the point $t\in\mathbb{RP}^1$ such that $\crochet{x,y;z,t}=-1$. For $\crochet{u(x),u(y);u(z),u(t)}$ to remain bounded, we must have $u(z)=u(t)$ and then again, $u$ has only 2 values.

\end{proof}

\subsection{The discrete approximations are uniformly quasi-symmetric.}



Recall that we started with a pair $(\lambda_-, \lambda_+)$  of laminations on $\HH^2$ that strongly fill. We associated to this pair:
\begin{itemize}
\item sequences $\lambda^n_\pm=\lambda^n_\pm$ of polyhedral pairs converging to $\lambda_\pm$, with $k_n$ vertices, and
\item a sequence of quasi-symmetric embeddings $v^n:\Z/k_n\Z\to\partial_\infty AdS^3$ such that $v^n_*(\lambda^n_\pm)$ are the measured bending laminations on the boundary of $CH(v^n(Z/k_n\Z))$.
\end{itemize}
%% We denote by $C_n=v^n(\mathbb{RP}^1)$. 

We then have a sequence of pairs of convex isometric embeddings $U^n_\pm:P^n_\pm\to AdS^3$, where $P^n_\pm$ are ideal polygons in $\HH^2$ with $k_n$ vertices, with images the upper and lower boundary components of $CH(v^n(\Z/k_n\Z))$. If we denote by $V_n$ the set of vertices of $P_\pm^n$ in $\partial_\infty\mathbb{H}^2$, we also consider the map $u^n_\pm=\partial U^n_\pm:V_n\subset \mathbb{RP}^1\rightarrow \partial_\infty AdS^3$. Those maps $u_\pm^n$ are injective and then have a left inverse $\left(u_\pm^n\right)^{-1}: \partial_\infty AdS^3\rightarrow \mathbb{RP}^1$. 


In order to apply \ref{lem:precompactness}, we need to show that the discrete maps $\left(u_\pm^n\right)^{-1}\circ v^n : \Z/k_n\Z \rightarrow \mathbb{RP}^1$ are \textit{uniformly} $(K,\epsilon)$-quasi-symmetric, in the sense of the previous paragraph. This is the point of the next lemma, whose proof uses decisively the fact that the laminations $\lambda^\pm$ are bounded.
%We know that the set of \textit{uniform} quasi-symmetric embeddings is compact \cite{lehtovirtanen}. That should be the main argument to obtain the quasi-circle. The uniform quasi-symmetric constants should in term follow from a uniform bound on the width on $C_n$:

\begin{lemma}
There exist $\epsilon>0$ and $K>1$ such that, for $n$ big enough, the maps $\left(u_\pm^n\right)^{-1}\circ v^n : \Z/k_n\Z \rightarrow \mathbb{RP}^1$ are $(K,\epsilon)$-quasi-symmetric.
\end{lemma}

\begin{remark}
In fact we can show the following equivalences ...\marginnote{L: I'm thinking of removing completely the width, even in the preliminaries}
\end{remark}

\begin{proof}
We argue by contradiction and we assume that the maps $f^n=\left(u_\pm^n\right)^{-1}\circ v^n$ are $(K_n,\varepsilon)$-quasi-symmetric with $K_n\to \infty$. We then have four sequences $(a_n), (b_n), (c_n)$ and $(d_n)$ in $\mathbb{RP}^1$ such that $\crochet{a_n,b_n;c_n,d_n}\in \crochet{1-\epsilon,1+\epsilon}$ and $\crochet{f^n(a_n),f^n(b_n);f^n(c_n),f^n(d_n)}\to 0$ (the case where $\crochet{f^n(a_n),f^n(b_n);f^n(c_n),f^n(d_n)}\to \infty$ is similar). Pre and post-composing by a Mobiüus map does not chnage the quasi-symmetry constant $K_n$. Hence, we may as well assume that $f^n$ sends $a_n=0,b_n=-1,c_n=\infty$ to $0,-1,\infty$ respectively and $f^n(d_n)$ converges to 0 (the normalization forces $d_n$ to be in the interval $\crochet{1-\epsilon, 1+\epsilon}$). We now (post) compose $f^n$ by a Mobiüs map $\gamma_n$ and we chose $\gamma_n$ such that it is a hyperbolic transformation whose repuslive fixed point is 0 and attractive fixed point is $\infty$. Representing $\gamma_n$ by a matrix in SL$_2(\mathbb{R})$, $\gamma_n$ has the form
\[
\gamma_n=\begin{pmatrix}
e^{\alpha_n} & 0\\
0 & e^{-\alpha_n}
\end{pmatrix},
\]
with $\alpha_n>0$ and $\alpha_n\to \infty$.
We want to choose the rate of attraction/repulsion $\alpha_n$ so that it provides a contradiction. We say that two sequences $(\alpha_n)$ and $(\alpha'_n)$ are uncomparable if either $\frac{\alpha_n}{\alpha'_n}\to 0$ or $\frac{\alpha_n}{\alpha'_n}\to +\infty$. Note that there is infinitely many uncomparable sequences and we will choose the sequence $\alpha_n$ among finitely many constraints.

First we require that $f^n\circ \gamma_n (d_n)$ tends to 0 and $f^n\circ\gamma_n(-d_n)$ tends to 0. Then, if we denote by $d_n^+$ the element of $ \Z/k_n\Z $ which is the successor of $d_n$ for the cyclic order on $\mathbb{RP}^1$ and $d_n^-$ the predecessor of $-d_n$ we choose $\alpha_n$ in such a way that $f^n\circ \gamma_n(d_n^-)$ and $f^n\circ \gamma_n (d_n^+)$ both tend to $\infty$.

Since the maps $f^n$ are increasing, we get that any element $x_n\in  \Z/k_n\Z $ which is in the interval $\crochet{-d_n,d_n}$ containing 0 satisfies $f^n\circ \gamma_n(x_n) \rightarrow 0$ and any element $x_n\in  \Z/k_n\Z $ in the interval $\crochet{d_n,-d_n}$ containing $\infty$ satisfies $f^n\circ \gamma_n(x_n)\rightarrow \infty$.

We conclude that the maps $u^n_\pm$ converge to the Rhombus curve constructed with the four points $a=-1, a'=1, b=\infty, b'=0$ (referring to the notation of paragraph \ref{subsec:rhombus}). The rhombus has two space-like geodesics inside $AdS^3$. Those geodesics bound lightlike planes and then both have an infinite dihedral angle, contradicting lemma \ref{lem:reciprocalbounds}.
\end{proof}


%\begin{lemma}
%The convex subsets $CH(v_n(\Z/k_n\Z))$ have width bounded away from $\frac{\pi}{2}$ (independent of $n$).
%\end{lemma}

%The proof is similar to one given, in a simular situation, in e.g. \cite{convexhull}.

%\begin{proof}
%  (outline)
  
%  (1) If not then after applying sequence of isometries, $x_-, x_+$ at time distance $\pi/2$.

%  (2) Support lines at $x_-$ and $x_+$, must be dual to each other because acausal meridian joining the vertices.

%  (3) The total bending near those two lines must go to infinity.

%  (4) Take four points $a,b,c,d$ separating the endpoints, e.g. vertices.

%  (5) Apply Lemma \ref{lem:reciprocalbounds}.
%\end{proof}

% \begin{proof}
% If not, the convex hull eventually (as $n\to\infty$) contains a rhombus.The rhombus has two space-like geodesics inside $AdS^3$. Those geodesics bound  lightlike planes and then both have an infinite dihedral angle, contradicting lemma \ref{lem:reciprocalbounds}.
% \end{proof}


%\subsection{The discrete approximations are uniformly quasi-symmetric}






\begin{lemma}
$(u^n_-)^{-1}\circ u^n_+$ is uniformly quasi-symmetric.
\end{lemma}

\begin{proof}
  
\end{proof}

%% NB the argument below might be useful, but they don't seem to be necessary.
% \begin{proof}
% Should follow from the fact that the projection \note{ref} from the upper to the lower boundary is a uniform quasi-isometry (which in turns should follow from the bound on the width).
% \end{proof}


%\begin{lemma}
%The homeomorphisms $(u^n_\pm)^{-1}\circ v^n$ are uniformly quasi-symmetric.
%\end{lemma}


%\begin{proof}
%We only treat the case of $(u^n_+)^{-1}\circ v_n$, the other one is obviously the same.
%We argue by contradiction and we suppose that the $(u^n_+)^{-1}\circ v_n$ are not uniformly quasi-symmetric. Then (?? check ??) there is a sequence of 4-tuples of points $(a_n,b_n,c_n,d_n)$ with images $(a'_n, b'_n, c'_n,d'_n)$ such that $cr(a_n,b_n,c_n,d_n)\geq n$ and $cr(a'_n,b'_n,c'_n,d'_n)\leq 1/n$. Because of the strong filling hypothesis, we can also assume for instance that $\lambda^n_+([a_n,b_n]\times [c_n,d_n])\geq n\epsilon/2$ (after extracting a subsequence). Indeed, choosing one of the two laminations, we can assume that $\lambda^n_+([a_n,b_n]\times [c_n,d_n])$ is the intersection number of a geodesic joining the arc $[a_n,d_n]$ to the arc $[b_n,c_n]$ which has length proportional to $n$. Then the upper boundary has bending measure going to $\infty$ near the geodesic which is the limit of the image of $(a'_n,b'_n)$ and $(c'_n, d'_n)$. Contradiction (with the fact that we don't have a "rhombus" in the limit.)
%\end{proof}

\subsection{Proof of Theorem \ref{tm:bending}}

Thanks to the lemma we can assume (after taking a subsequence and normalizing by M\"obius transformations) that the $(u^n_\pm)^{-1}\circ v^n$ are converging to quasi-symmetric homeomorphisms. It should then follow that the sequence of convex pleated surfaces converge and that the bending lamination on the boundary converges to $\lambda_+, \lambda_-$.
